On the Structures of Representation for the Robustness of Semantic Segmentation to Input Corruption

Semantic segmentation is a scene understanding task at the heart of safety-critical applications where robustness to corrupted inputs is essential. Implicit Background Estimation (IBE) has demonstrated to be a promising technique to improve the robustness to out-of-distribution inputs for semantic segmentation models for little to no cost. In this paper, we provide analysis comparing the structures learned as a result of optimization objectives that use Softmax, IBE, and Sigmoid in order to improve understanding their relationship to robustness. As a result of this analysis, we propose combining Sigmoid with IBE (SCrIBE) to improve robustness. Finally, we demonstrate that SCrIBE exhibits superior segmentation performance aggregated across all corruptions and severity levels with a mIOU of 42.1 compared to both IBE 40.3 and the Softmax Baseline 37.5.

==> _1_figures/allcorruptions.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{_3_images/corruption_ex.png}
\centering
\caption{Examples of five corruptions across five severity levels from \cite{hendrycks2018benchmarking} for an image from PASCAL VOC 2012 \cite{EveringhamPascalVisualObject2015}.}
\label{fig:corrsum}
\end{figure}

==> _4_sections/_2_related_work.tex <==
\section{Related Work}
\label{sec:related}
Robustness for deep vision involves circumstances where erroneous predictions are caused by some invalid input---more specifically: out-of-distribution (OOD), adversarial, or corrupted. 
The two directions for recovery when faced with an invalid input are to maintain nominal behavior (corrupted or adversarial) or detect (all).

\smpar{OOD} In the case of OOD for image classification, it is impossible to maintain nominal behavior when the representation is inadequate to handle the complement of in-distribution inputs e.g. a 3-class classifier that predicts between dog, cat, and bird can never predict platypus.
Designing OOD detectors has been an active direction in image classification \cite{hendrycks17baseline, hendrycks2018oe, guo2017calibration, liang2018enhancing, lee2018training, lee2018simple}.
In particular, the baseline detector proposed by \cite{hendrycks17baseline} can be applied to any image classifier as well as semantic segmentation model. 
As was demonstrated in \cite{lehman2019implicit}, semantic segmentation models have the additional benefit of performing nominally in the face of an OOD input by way of the background class.

\smpar{Adversarial} Adversarial inputs are manufactured to elicit a particular model response.
Characterized as attacks, these techniques can be applied to modify images in ways imperceptible to humans that are still effective against a target model \cite{GoodfellowExplainingharnessingadversarial2014, papernot2016limitations, Carlinievaluatingrobustnessneural2017}.
Defending against attacks can involve detection \cite{}

For semantic segmentation, \cite{arnab2018robustness} 

\smpar{Corrupted} Of the three, corrupted inputs cover a broad range of invalid inputs.


broad category  


==> _5_misc/ibe.tex <==
\smpar{Implicit Background Estimation}
When background is a class that must be learned---as with VOC2012---a problem arises with neglecting negative detection and requiring a fully connected dependency.
Background is the complement of the foreground classes.
In the case of VOC2012, the model must learn to represent potentially $k-1$ representations for background---one for each foreground class.
As was demonstrated in \cite{lehman2019implicit} and shown on the right of Figure \ref{fig:wholeflow}, by restricting detection of the background class to when all of the foreground components, $\vect{v}_{FG}\in\R^{k-1}$ are all in the negative orthant of $\R^{k-1}$, the surjections of Softmax are eliminated. 
Also, by inspecting the gradient update for IBE

\vspace{-1.5em}
\begin{align}
\label{eq:smibe_grad}
    \frac{\delta L}{\delta v_{i,j,n}} =  \begin{cases}
    -\frac{2 e^{v_{i,j,n}} \sum_{\text{FG}}e^{v_{i,j,m}} } {(\sum_{\text{FG}}e^{v_{i,j,m}})^2+1} \qquad n = \text{Background}&\\
    \softmax_{SM}(\vect{v}_{i,j})^{(n)} - y_{i,j,n} \qquad n \in \text{Foreground}&
    \end{cases}
\end{align}

we can see that the TN and FN components for foreground classes are reinforced when the background is updated.
This is again evident in Figure \ref{fig:autocorrelation}, where for both IBE and SCrIBE, there is orthogonality evident between component $13$ and all other components.
The outcome of this reinforcement will decorrelate TP detections allowing for the observed improvements in calibration and out-of-distribution detection in \cite{lehman2019implicit}.
However, as Softmax is still in use, the structure retains fully connected dependence for the foreground, and a binary dependence between the foreground classes and the shared background class.
This structure is depicted in Figure \ref{fig:dependence}.

==> _5_misc/preliminaries.tex <==
\smpar{Preliminaries} Let a semantic segmentation model be, $f(x):\R^{H\times W\times 3}\rightarrow \R^{H\times W \times k}$ and at each pixel location the output of $f(x)$ is $\vect{v}_{i,j}\in\R^k$, where $k$ is the number of classes.
$f(x)$ learns a representation for $\vect{v}_{i,j}$, which we define as $\K\in\R^k$. 
Also defined at each pixel is a categorical label, $\vect{y}_{i,j}$, as a one-hot vector.
Let softmax be, $\softmax_{SM}(\vect{x})$ and sigmoid be, $\softmax(\vect{x})$.

==> _5_misc/scribe.tex <==



==> _5_misc/sigmoid.tex <==

\smpar{Sigmoid}
To give some context on why Sigmoid is a poor choice for categorical classification consider the gradient update at $i,j$
    
\vspace{-1.5em}
\begin{align}
\label{eq:sg_grad}
    \frac{\delta L}{\delta v_{i,j,n}} = -y_{i,j,n}(1-\softmax(v_{i,j,n})).
\end{align}
\vspace{-1em}

\noindent
Notice that this penalizes only for FN.  
Additionally, it allows for undesirable cases where $\vect{v}_{i,j}$ is a collection of large positive values---driving the $1-\softmax(\vect{v}_{i,j,n})$ term to 0---resulting in no gradient updates regardless the value of $y_{i,j,n}$. 
However, the key difference from Softmax that we will utilize is that Sigmoid "pins" component responses about 0, eliminating the relative dependence inherent with Softmax resulting in a structure of $k$ independent binary detectors.

==> _5_misc/softmax.tex <==

\smpar{Softmax}
Consider a model trained with Softmax Cross Entropy that achieves satisfactory task performance.
Beginning with the definition for the gradient of the Softmax Cross Entropy Loss for Semantic Segmentation in \eqref{eq:sm_grad}.  Let $\vect{x}^{(n)}$ be the scalar value of a vector indexed at $n$.

\vspace{-2em}
\begin{align}
\label{eq:sm_grad}
    \frac{\delta L}{\delta v_{i,j,n}} = \softmax_{SM}(\vect{v}_{i,j})^{(n)} - y_{i,j,n}.
\end{align}

During training, the updates follow the pattern of reinforcing True Positives (TP) by making that component larger and positive,  reinforcing True Negatives (TN) by making those components larger and negative, and punishing False Positives (FP) and False Negatives (FN) in the opposite way.
Though this behavior is desirable, Softmax heavily favors reinforcing TP and punishing FP because the updates for FN and TN depend on the relative magnitude of the components in $\vect{v}_{i,j}$ where $y_{i,j,n}=0$.
One insight is that those components associated with negative detection are neglected in optimization---moreso as $k$ increases.
This is evident in Figure \ref{fig:autocorrelation}, where the Baseline exhibits a chaotic structure in the autocorrelation of $\vect{v}_{i,j}^{13}$ because throughout training the FN and TN components were neglected leaving them close to the responses at initialization.
Another insight is that the structure of optimization depends only on the relative response in $\vect{v}_{i,j}$.
This structure is fully connected because detection depends on every component as shown for the Baseline in Figure \ref{fig:dependence}.




